Contrastive Deep Learning Reveals Age Biomarkers in Histopathological Skin Biopsies

As global life expectancy increases, so does the burden of chronic diseases, yet individuals exhibit considerable variability in the rate at which they age. Identifying biomarkers that distinguish fast from slow ageing is crucial for understanding the biology of ageing, enabling early disease detection, and improving prevention strategies. Using contrastive deep learning, we show that skin biopsy images alone are sufficient to determine an individual's age. We then use visual features in histopathology slides of the skin biopsies to construct a novel biomarker of ageing. By linking with comprehensive health registers in Denmark, we demonstrate that visual features in histopathology slides of skin biopsies predict mortality and the prevalence of chronic age-related diseases. Our work highlights how routinely collected health data can provide additional value when used together with deep learning, by creating a new biomarker for ageing which can be actively used to determine mortality over time.

==> 01_abstract.tex <==
Ageing is associated with progressive structural and cellular remodelling across tissues, yet individuals of similar chronological age exhibit substantial heterogeneity in disease burden and survival. Identifying biomarkers that capture biological aspects of ageing beyond chronological age remains a major challenge. Here, we investigated whether routine skin histopathology contains latent ageing-associated morphological information linked to long-term health outcomes.

We analysed digitised skin biopsy whole-slide images from 1,787 individuals linked to nationwide Danish health registries containing demographic information, disease diagnoses, and mortality follow-up. Using contrastive self-supervised deep learning, we extracted high-dimensional histological feature representations from multiscale skin biopsy image patches and generated morphology-derived histological age estimates. Histological age acceleration was subsequently defined as the deviation between histological and chronological age.

Histological age estimates correlated strongly with chronological age and captured biologically interpretable tissue features associated with skin ageing, including epidermal atrophy, collagen degeneration, altered dermal organisation, and inflammatory disruption. Histological age acceleration consistently improved discrimination of prevalent age-related diseases relative to chronological age alone and remained independently associated with elevated long-term mortality risk in sex-stratified survival analyses. Unsupervised clustering of learned feature representations further revealed progressive transitions from preserved tissue architecture toward increasingly degraded ageing-associated morphology.

Together, these findings demonstrate that routine skin histopathology contains clinically relevant ageing-associated tissue signatures linked to disease burden and survival. More broadly, this work highlights the potential of combining large-scale pathology archives, national health registries, and self-supervised deep learning to derive morphology-based biomarkers of human ageing from routinely collected clinical data. \\

\textbf{Keywords:} Histological age, self-supervised learning, computational pathology, skin biopsy

==> 01_big_picture.tex <==

\section*{Highlights}

\begin{itemize}
    \item Self-supervised contrastive learning identified ageing-associated morphology in routine skin histology.
    \item Histological feature representations generated morphology-derived age estimates from digitised skin biopsies.
    \item Histological age acceleration was associated with age-related disease burden and long-term mortality.
    \item Dimensionality reduction and clustering analyses revealed biologically interpretable ageing-associated tissue patterns.
    \item Routine pathology archives may provide scalable digital biomarkers for biological ageing research.
\end{itemize}

\section*{Summary}





==> 09_consent.tex <==
\subsection*{Consent for publication}

Not applicable.

\subsection*{Ethics approval and consent to participate}

Not applicable.
